Election algorithms with random delays in trees

The election is a classical problem in distributed algorithmic. It aims to design and to analyze a distributed algorithm choosing a node in a graph, here, in a tree. In this paper, a class of randomized algorithms for the election is studied. The election amounts to removing leaves one by one until the tree is reduced to a unique node which is then elected. The algorithm assigns to each leaf a probability distribution (that may depends on the information transmitted by the eliminated nodes) used by the leaf to generate its remaining random lifetime. In the general case, the probability of each node to be elected is given. For two categories of algorithms, close formulas are provided.

==> header.tex <==
\pagestart{611}

\pageend{622}
\authorhead{Jean-Fran{\c c}ois Marckert  and Nasser Saheb-Djahromi and Akka Zemmari}
\titlehead{Election with delays in trees}
\keywords{\relax }


